KRust: A Formal Executable Semantics of Rust

Rust is a new and promising high-level system programming language. It provides both memory safety and thread safety through its novel mechanisms such as ownership, moves and borrows. Ownership system ensures that at any point there is only one owner of any given resource. The ownership of a resource can be moved or borrowed according to the lifetimes. The ownership system establishes a clear lifetime for each value and hence does not necessarily need garbage collection. These novel features bring Rust high performance, fine low-level control of C and C++, and unnecessity in garbage collection, which differ Rust from other existing prevalent languages. For formal analysis of Rust programs and helping programmers learn its new mechanisms and features, a formal semantics of Rust is desired and useful as a fundament for developing related tools. In this paper, we present a formal executable operational semantics of a realistic subset of Rust, called KRust. The semantics is defined in K, a rewriting-based executable semantic framework for programming languages. The executable semantics yields automatically a formal interpreter and verification tools for Rust programs. KRust has been thoroughly validated by testing with hundreds of tests, including the official Rust test suite.

==> applications.tex <==
\section{Applications}
Here we describe applications of our formal Rust semantics, which are automatically derived from the semantics. As we have introduced, our formal Rust semantics are implemented by K, which is a rewriting-logic(RL) \cite{Mes92} executable semantic framework. Through this, our applications are essentially wrappers, or views, of the semantics, not needing to  develop a different model for each application tool.

\subsection{Interpreter}
Through the RL, we can find that evolution of a program can be clearly described using rewrite rules when we use RL formalise semantics for language, which will yield a transition system for any program. The semantics yields an interpreter called $\krust$,  we can use $\krust$ to run Rust test cases. Besides, we can use $\krust$ to help us to validate our semantics.

\subsection{Compiler Testing}
Compilers are widely used software in today's world. the correctness of the compilers is very important for us. So in last years, people mainly proposed three compiler testing methods:Randomized Differential Testing (RDT) \cite{mckeeman1998differential, sheridan2007practical, yang2011finding, chen2016empirical}, a variant of RDT|Different Optimization Levels (DOL) \cite{sheridan2007practical, chen2016empirical}, and Equivalence Modulo Inputs (EMI)\cite{le2014compiler, chen2016empirical}.And people have found a lot of compiler crash and compiler miscompilation problems in GCC,LLVM and other compilers. For Rust compiler, we don't know whether there exists compiler crash and compiler miscompilation problems. Now when we have KRust, we can carry on Rust compiler testing by RDT method through the comparison with the original Rust compiler.

RDT is a widely-used compiler testing technique, which addresses the test oracle problem in compiler testing using two or more comparable compilers that implement the same specification. Because these comparable
compilers should produce the same results under the same set of test inputs, it is easy for us to determine whether compilers contain bugs. That is, if any two compilers generate different results, there will exist bugs in one of the compilers. For detail, when given a set of compilers under test, denoted as $\{C_1,C_2,....,C_n\}$, and $n\geq 2$, the process for applying RDT to test these compilers is as follows. Each compiler $C_i$ compiles a test program P and generates an executable $E_i$, where $ 1\leq i \leq n$. For any given set of test inputs for P, denoted as I, these executables produce different results, denoted as
$O_1, O_2, ..., O_n$. Because the compilers under test are designed to follow the same specification, their behaviors are expected to be the same. Therefore, RDT detects compiler bugs through comparison among $O_1, O_2, ..., O_n$.

For Rust compiler testing, we can use our KRust and original Rust compiler, these two are implemented by the same Rust semantics specification, then follow the methods we introduced in RDT: we can choose Rust test program \emph{P}, compiled by KRust and original Rust compiler, then given the same input \emph{I}, if the executable results are different, we can know there may exists bugs in KRust or original Rust compiler, if we can make sure our semantics are re-write correctly by K, then we may know there exists bugs in original Rust compiler.

%\subsection{Runtime Verification(Catching undefined behavior)(Symbolic Execution)}






==> limitations.tex <==
\section{Limitations}

